PhraseCut: Language-based Image Segmentation in the Wild

We consider the problem of segmenting image regions given a natural language phrase, and study it on a novel dataset of 77,262 images and 345,486 phrase-region pairs. Our dataset is collected on top of the Visual Genome dataset and uses the existing annotations to generate a challenging set of referring phrases for which the corresponding regions are manually annotated. Phrases in our dataset correspond to multiple regions and describe a large number of object and stuff categories as well as their attributes such as color, shape, parts, and relationships with other entities in the image. Our experiments show that the scale and diversity of concepts in our dataset poses significant challenges to the existing state-of-the-art. We systematically handle the long-tail nature of these concepts and present a modular approach to combine category, attribute, and relationship cues that outperforms existing approaches.

==> experiment_old.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Region proposal performance}
\label{sec:exp-proposal}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/proposal_m.pdf}
\end{center}
\vspace{-0.15in}
   \caption{\textbf{Region proposal upper-bound performance.}
   We report the box/mask mean IoU of picking the best one among top $k$ candidate regions.}
\label{fig:exp-propsal}
\vspace{-0.1in}
\end{figure}

We use detected instances from Mask-RCNN trained on our dataset as the region candidates. Detected instances are ranked by their objectness scores.
Given a phrase-region query task, we calculate the upper-bound performance when picking the best region among the top $k$ candidates by picking the one with maximum IoU against the ground-truth target region. 
We evaluated the mean IoU of both masks (candidate mask vs. ground-truth mask) and boxes (candidate box vs. the union of all ground-truth instance boxes.)
Figure~\ref{fig:exp-propsal} presents the result on the validation set.
Note that the ground truth region only consists of one or very few instances, while Mask-RCNN tries to detect all the instances.
We can see that with the increment of $k$, the curve grows fast and soon gets relatively steady. 
The top $15$ candidates get an upper-bound IoU over $0.5$, meaning that on average, we can get a roughly correct box within the top $15$ candidates, which validates the effectiveness of our trained MaskRCNN model.
The curve becomes steady after top $50$, so we choose to use the top $50$ candidates as the input to the following comprehension stage.
\vspace{-0.1in}
\paragraph{Quality of Visual Genome boxes} 
Given a phrase, we select Visual Genome boxes that matches all of the category names, attributes and relationship descriptions in the phrase as the predicted boxes, and compute its mean box IoU against ground-truth instance boxes collected in our dataset.
This can be viewed as an examination of Visual Genome box qualities, because we originally generated the phrases from annotations on Visual Genome boxes, and ask users to label the corresponding region, now we compare original Visual Genome boxes with human input as the ground-truth. 
Visual Genome boxes only get a mean IoU of $0.474$, which is similar as the upper-bound of top $10$ candidates from Mask-RCNN as shown in Figure~\ref{fig:exp-propsal}.
This proves that 
(1) Visual Genome boxes are noisy and it is necessary to collect region annotations from the human. 
(2) Mask-RCNN trained on our dataset is a good region proposal model. 


\begin{table}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l||c|c|c|c|c|}
\hline
Model             & mean-IoU & cum-IoU & Pr@0.5  & Pr@0.7 & Pr@0.9 \\
\hline\hline
obj+cat &0.409 &0.434	&0.427		&0.290	&0.050 \\
obj+cat+att &0.417	&0.451	&0.438		&0.301	&0.055 \\
obj+cat+match &0.416	&0.448	&0.436		&0.299	&0.053 \\
obj+cat+[sub,loc,rel] &0.421	&0.454	&0.445	&0.305		&0.055 \\
obj+cat+match+att  &0.414	&0.443	&0.434		&0.296		&0.052 \\
obj+cat+[sub,loc,rel]+att &0.423	&0.457	&0.448	&0.307		&0.057 \\
obj+cat+[sub,loc,rel]+att:thresh &\textbf{0.445}	&\textbf{0.462}	&\textbf{0.469}		&\textbf{0.310}		&\textbf{0.062} \\
\hline
RMI  &0.203	 &0.419	&0.211	&0.109	&0.014\\
MattNet &0.201	&0.223	&0.193		&0.132 &0.028 \\
Mask-RCNN:top cat  &0.355	&0.386	&0.363	&0.255		&0.051 \\
Mask-RCNN:upper-bound   &0.610 &	0.677 &	0.689 &	0.480&		0.106 \\
\hline
\end{tabular}}
\end{center}
\caption{Ablation study and comparisons with baseline methods.}
\vspace{-0.1in}
\label{tab:exp-result}
\end{table}

% \begin{table}
% \begin{center}
% \resizebox{1.05\linewidth}{!}{
% \begin{tabular}{|l||c|c|c|c|c|c|c|}
% \hline
% Model             & mIoU & cIoU & Pr@0.5 & Pr@0.6 & Pr@0.7 & Pr@0.8 & Pr@0.9 \\
% \hline\hline
% obj+cat &0.4092 &0.4337	&0.4274	&0.3637	&0.2899	&0.1912	&0.0497 \\
% obj+cat+att &0.4170	&0.4512	&0.4383	&0.3757	&0.3009	&0.2004	&0.0545 \\
% obj+cat+match &0.4155	&0.4482	&0.4362	&0.3734	&0.2990	&0.1980	&0.0533 \\
% obj+cat+[sub,loc,rel] &0.4207	&0.4537	&0.4445	&0.3805	&0.3047	&0.2024	&0.0553 \\
% obj+cat+match+att  &0.4139	&0.4434	&0.4344	&0.3708	&0.2959	&0.1957	&0.0517 \\
% obj+cat+[sub,loc,rel]+att &0.4229	&0.4574	&0.4476	&0.3836	&0.3074	&\textbf{0.2052}	&0.0567 \\
% obj+cat+[sub,loc,rel]+att:th &\textbf{0.4445}	&\textbf{0.4619}	&\textbf{0.4690}	&\textbf{0.3935}	&\textbf{0.3098}	&0.2044	&\textbf{0.0623} \\
% \hline
% RMI  &0.2032	 &0.4185	&0.2110	&0.1600	&0.1089	&0.0586	&0.0143\\
% MattNet &0.2008	&0.2230	&0.1926	&0.1634	&0.1321	&0.0897	&0.0284 \\
% Mask-RCNN:top cat  &0.3547	&0.3858	&0.3627	&0.3133	&0.2546	&0.1733	&0.0511 \\
% Mask-RCNN:upper-bound   &0.6103 &	0.6769 &	0.6892 &	0.5932 &	0.4797 &	0.3223 &	0.1060 \\
% \hline
% \end{tabular}}
% \end{center}
% \caption{Ablation study and comparison with baselines on the full test set.}
% \label{tab:exp-result}
% \end{table}


\begin{table*}
\begin{center}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{|l||c c|c | c|c c|c c|}
\hline
Model  & att+ & rel+  & 101-500   & multi  & large & small & stuff & obj\\ 
\hline\hline
obj+cat &0.379	&0.295	&0.366	&0.303	&0.543	&\textbf{0.276}	&0.433	&0.388 \\
obj+cat+att 	&0.383	&0.302	&0.369	&0.309	&0.564	&0.276	&0.445	&0.393   \\
obj+cat+match &0.382	&0.305	&0.368	&0.308	&0.559	&0.276	&0.442	&0.392  \\
obj+cat+[sub,loc,rel] 	&0.389	&0.320	&0.372	&0.312	&0.573	&0.275	&0.449	&0.396  \\
obj+cat+match+att 	&0.380	&0.299	&0.368	&0.306	&0.554	&0.276	&0.439	&0.392   \\
obj+cat+[sub,loc,rel]+att 	&0.389	&0.314	&0.374	&0.315	&0.581	&0.274	&0.452	&0.398 \\
obj+cat+[sub,loc,rel]+att:thresh	&\textbf{0.412}	&\textbf{0.346}	&\textbf{0.387}	&\textbf{0.381}	&\textbf{0.647}	&0.265	&\textbf{0.477}	&\textbf{0.417}  \\
\hline
RMI  &0.207	&0.113	&0.128	&0.156	&0.491	&0.013	&0.278	&0.138      \\
MattNet 	&0.188	&0.159	&0.141	&0.153	&0.398	&0.064	&0.239	&0.167     \\
Mask-RCNN:top cat &0.326	&0.257	&0.300	&0.252	&0.493	&0.208	&0.385	&0.328  \\
Mask-RCNN:upper-bound &0.642	&0.598	&0.583	&0.478	&0.761	&0.435	&0.635	&0.589      \\
\hline
\end{tabular}}
\end{center}
\caption{\textbf{Mean IoU on selected subsets.}
The subsets follow the same definition as in Figure~\ref{fig:data_stat}. att+(rel+): the subset in which attribute (relationship) is required to distinguish target instances from others of the same category.101-500: category frequency ranked between 101 and 500. multi: referring to multiple instance with one phrase. large/small: target region is greater than $20\%$ / below $2\%$ of the image area. stuff/obj: background stuff or foreground object.}
\label{tab:exp-subtask}
\vspace{-0.05in}
\end{table*}

\begin{figure*}
\begin{center}
   \includegraphics[width=0.8\linewidth]{figures/result.pdf}
\end{center}
\vspace{-0.1in}
   \caption{\textbf{Prediction results on \vgp dataset.} Columns from left to right are: (1) ground-truth segmentation and instance boxes; (2) Candidate boxes from Mask-RCNN (randomly showing $10$ boxes out of $50$ candidates) and segmentation of the best candidate; (3) Mask-RCNN baseline with top1 category score as the prediction; (4) MattNet baseline; (5) RMI baseline: it outputs empty mask in the third example; (5) Our best model.}
\label{fig:exp-example}
\vspace{-0.15in}
\end{figure*}



\subsection{Comparison of models}
We run experiments on baseline models of Mask-RCNN, MattNet and RMI as introduced in Section~\ref{sec:method}.
The full version of our proposed three-stage model takes $9$ input numbers in the final ensemble: the objectness and category scores from Mask-RCNN, the attribute score from MattNet, as well as the three pairs of modular scores and weights from the subject, location and relationship modules in MattNet.
We also carry out a series of ablation study as listed in Table~\ref{tab:exp-result} and \ref{tab:exp-subtask}.
Table~\ref{tab:exp-result} shows the statistics on the overall test split; Table~\ref{tab:exp-subtask} displays mean IoU on subsets.
Figure~\ref{fig:exp-example} shows example prediction results.

MattNet and RMI report good results on MS-COCO based referring datasets, but do not perform as well on our \vgp dataset.
They get Pr@0.7 of $67.83\%$ and $22.75\%$ respectively on RefCOCO validation set, but only get $13.21\%$ and $10.89\%$ on our dataset.
MattNet and RMI are similar in terms of overall mean IoU ($0.2008$ vs, $0.2032$), 
but RMI gets a suspicious high cum-IoU of $0.4185$ which doesn't match with the quality of its visualization results.
This is because RMI works well on larger regions and background stuff, which are dominating cum-IoU.
On the other hand, MattNet performs better than RMI on tail categories, smaller regions, and relationships.

We show that picking the instance with top category score in pure Mask-RCNN is a surprisingly strong baseline.
It exceeds MattNet and RMI by a large margin, especially on medium sizes, foreground objects and the ``category+" subset. 
Limited by the category classifier trained for instance detection, it is relatively weak on ``att+", ``rel+" subsets and also regions that are too small or large.

From Mask-RCNN's upper-bound performance on different subsets, we notice that the performance on multi-instance and small size are lower than rest subsets. Low in multi-instance is reasonable as we always choose the top-$1$ candidate.
Low in small-sized regions indicates that Mask-RCNN performs worse on smaller instances.

Our experiments show that adding the third ensemble stage is very beneficial for model performance.
By learning only $10$ additional weights, Mask-RCNN (mean IoU=$0.3547$) and MattNet(meanIoU=$0.2008$) are combined into a high performance model if mean IoU=$0.4445$.

The first improvement comes from a linear ensemble. A simple linear combination of objectness and category scores pushes the mean IoU from $0.3547$ to $0.4092$.
Adding MattNet to the input improves mean IoU from $0.4092$ to $0.4229$ with better performance on the challenging ``rel+" subset and also the simpler subsets of ``stuff" and ``large" regions which are not the strength of Mask-RCNN. 
Finally, adding the relative thresholding scheme improves the performance to $0.4445$, improving mean IoU in ``multi" and ``many" instance subsets, as well as the ``large" region category.

We show that using internal modular scores and weights of MattNet gives better performance than just the single final matching score from MattNet. 
We, therefore, argue that ensemble with signals from region proposal in the loop is better than combining modular scores with weights only based on query phrases. We also discover the effect of adding attribute scores is more obvious for ``top 100" categories, ``large" regions and ``stuff" instead of ``att" and ``att+" subset. 
Our interpretation is that the current model weighs more on categories and attribute scores only help when the category is simple to predict.


\subsection{Analysis on subsets}

Our results indicate that background stuff is simpler than foreground objects and they can be handled within the same pipeline.
Small regions are extremely challenging, and we lose a lot of accuracy during the region proposal stage. The best model so far on ``small" regions is a simple ensemble of objects and category score from Mask-RCNN. MattNet and RMI encounter total failure in the ``small" region subset.
Correlated with ``small" regions, less frequent categories are also challenging and suffering in the region proposal stage.
Multi-region referral is improved by relative thresholding but is still far from being solved. 
There is also a large room of improvement on attributes and relationships that call further study into them.

\vspace{-0.15\baselineskip}


% \begin{table}[t]
% 	\begin{center}
% 		\resizebox{\linewidth}{!}{
% 			\begin{tabular}{|l||c|c|c|c|c|c|}
% 				\hline
% 				Subset & \% of data & box acc &  IoU$_b$ & acc$_b$@0.5 & acc$_b$@0.7 & acc$_b$@0.9 \\
% 				\hline\hline
% 				overall & 10,937 & &0.54 & &0.58 & &0.56 & &0.49 & &0.42 \\
% 				att & 5,265 & &0.56 & &0.61 & &0.59 & &0.53 & &0.47 \\
% 				dist-att & 1,358 & &0.41 & &0.53 & &0.51 & &0.45 & &0.37 \\
% 				rel & 1,535 & &0.46 & &0.50 & &0.49 & &0.41 & &0.33 \\
% 				dist-rel & 254 & &0.31 & &0.40 & &0.39 & &0.32 & &0.23 \\
% 				rare & 211 & &0.32 & &0.37 & &0.35 & &0.32 & &0.27 \\
% 				multi & 1,836 & &0.44 & &0.48 & &0.45 & &0.35 & &0.26\\
% 				\hline
% 		\end{tabular}}
% 	\end{center}
% 	\label{tab:subset}
% 	\caption{\todo{should report on our best model. This MattNet result is on old val/test split. }Performance of MattNet on subsets. We report the box accuracy (picking the right box), average IoU with the ground-truth referred instance box(es), and the accuracy with IoU above a threshold of $0.5, &0.7, &0.9$.}
% \end{table}


